Measurement of $\Sigma^+$ transverse polarization in $e^+e^-$ collisions at $\sqrt{s} = 3.68-3.71$ GeV

Using $e^+e^-$ collision data collected with the BESIII detector at seven energy points ranging from 3.68 to 3.71 GeV and corresponding to an integrated luminosity of $652.1~{\rm pb^{-1}}$, we present an energy-dependent measurement of the transverse polarization, relative phase and modulus ratio of the electromagnetic form factors of the $\Sigma^+$ hyperon in the $e^+e^- \to \Sigma^+ \bar{\Sigma}^-$ reaction. These results are helpful to understand the production mechanism of the $\Sigma^+$-$\bar\Sigma^-$ pairs.

==> def-com.tex <==

%%************************************************************
%% Shared ones
%%************************************************************
\newcommand{\BR}{\mathcal{B}}
\newcommand{\afs}{\alpha_s}
\newcommand{\bgp}{\beta\gamma}
\newcommand{\eff}{\varepsilon}
\newcommand{\sintht}{\sin{\theta}}
\newcommand{\costht}{\cos{\theta}}
%\newcommand{\Npsp}{N_{\psi(2S)}}
\newcommand{\dedx}{dE/dx}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%event selection
\newcommand{\probfc}{Prob_{\chi^2}}
\newcommand{\probpi}{Prob_{\pi}}
\newcommand{\probka}{Prob_{K}}
\newcommand{\probpr}{Prob_{p}}
\newcommand{\proball}{Prob_{all}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%charmonium
\newcommand{\chicJ}{\chi_{cJ}}
\newcommand{\gchicJ}{\gamma\chi_{cJ}}
\newcommand{\gchica}{\gamma\chi_{c0}}
\newcommand{\gchicb}{\gamma\chi_{c1}}
\newcommand{\gchicc}{\gamma\chi_{c2}}
\newcommand{\hc}{h_c(^1p_1)}
\newcommand{\qqb}{q\bar{q}}
\newcommand{\uub}{u\bar{u}}
\newcommand{\ddb}{d\bar{d}}
\newcommand{\BBb}{B\bar{B}}
\newcommand{\BB}{B\bar{B}}
\newcommand{\ccb}{c\bar{c}}
%\newcommand{\ppb}{p\bar{p}}
\newcommand{\llb}{\Lambda\bar{\Lambda}}
\newcommand{\LcLcB}{\Lambda_c^+\bar{\Lambda}_c^-}
\newcommand{\ssb}{\Sigma^{0}\bar\Sigma^{0}}
\newcommand{\SSB}{\Sigma^+\bar{\Sigma}^-}
\newcommand{\XXN}{\Xi^{0}\bar\Xi^{0}}
\newcommand{\XXB}{\Xi^{-}\bar\Xi^{+}}
\newcommand{\SSSN}{\Sigma(1385)^{0}\bar\Sigma(1385)^{0}}
\newcommand{\SSSM}{\Sigma(1385)^{-}\bar\Sigma(1385)^{+}}
\newcommand{\SSSP}{\Sigma(1385)^{+}\bar\Sigma(1385)^{-}}
\newcommand{\SSPM}{\Sigma(1385)\bar\Sigma(1385)}
\newcommand{\XXXB}{\Xi(1530)^{-}\bar\Xi(1530)^{+}}
\newcommand{\XXXM}{\Xi(1530)^{0}\bar\Xi(1530)^{0}}
\newcommand{\XXBB}{\Xi(1530)^{-}\bar\Xi^{+}}
\newcommand{\XXBBCC}{\Xi(1530)^{-}\bar\Xi^{+}+c.c.}
\newcommand{\XXNN}{\Xi(1530)^{0}\bar\Xi^{0}+c.c.}



%%************************************************************
%% Variables: decay modes of psiprime
%%************************************************************
\newcommand{\psipto}{\psi(2S)\rightarrow \pi^+\pi^- J/\psi}
\newcommand{\ptomm}{J/\psi\rightarrow \mu^+\mu^-}
\newcommand{\ppp}{\pi^+\pi^- \pi^0}
\newcommand{\pip}{\pi^+}
\newcommand{\pim}{\pi^-}
%\newcommand{\pi0}{\pi^0}
\newcommand{\kap}{K^+}
\newcommand{\kam}{K^-}
\newcommand{\ks}{K^0_s}
\newcommand{\pbar}{\bar{p}}
\newcommand{\jp}{J/\psi\rightarrow \gamma\pi^0}
\newcommand{\je}{J/\psi\rightarrow \gamma\eta}
\newcommand{\jec}{J/\psi\rightarrow \gamma\eta_{c}}
\newcommand{\jep}{J/\psi\rightarrow \gamma\eta^{\prime}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 2prongs
\newcommand{\LL}{\ell^+\ell^-}
\newcommand{\EE}{e^+e^-}
\newcommand{\MM}{\mu^+\mu^-}
\newcommand{\GG}{\gamma\gamma}
\newcommand{\TT}{\tau^+\tau^-}
\newcommand{\pp}{\pi^+\pi^-}
\newcommand{\kk}{K^+K^-}
\newcommand{\ppb}{p\bar{p}}
\newcommand{\gpp}{\gamma \pi^+\pi^-}
\newcommand{\gkk}{\gamma K^+K^-}
\newcommand{\gppb}{\gamma p\bar{p}}
\newcommand{\ggee}{\gamma\gamma e^+e^-}
\newcommand{\gguu}{\gamma\gamma\mu^+\mu^-}
\newcommand{\ggll}{\gamma\gamma l^+l^-}
\newcommand{\ppee}{\pi^+\pi^- e^+e^-}
\newcommand{\ppuu}{\pi^+\pi^-\mu^+\mu^-}
\newcommand{\etap}{\eta^{\prime}}
\newcommand{\gpi}{\gamma\pi^0}
\newcommand{\geta}{\gamma\eta}
\newcommand{\getap}{\gamma\etap}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 4prongs
\newcommand{\pppp}{\pi^+\pi^-\pi^+\pi^-}
\newcommand{\ppkk}{\pi^+\pi^-K^+K^-}
\newcommand{\pppr}{\pi^+\pi^-p\bar{p}}
\newcommand{\kkkk}{K^+K^-K^+K^-}
\newcommand{\kskp}{K^0_s K^+ \pi^- + c.c.}
\newcommand{\ppkp}{\pi^+\pi^-K^+ \pi^- + c.c.}
\newcommand{\ksks}{K^0_s K^0_s}
\newcommand{\dphi}{\phi\phi}
\newcommand{\phikk}{\phi K^+K^-}
\newcommand{\ppeta}{\pi^+\pi^-\eta}
\newcommand{\gpppp}{\gamma \pi^+\pi^-\pi^+\pi^-}
\newcommand{\gppkk}{\gamma \pi^+\pi^-K^+K^-}
\newcommand{\gpppr}{\gamma \pi^+\pi^-p\bar{p}}
\newcommand{\gkkkk}{\gamma K^+K^-K^+K^-}
\newcommand{\gkskp}{\gamma K^0_s K^+ \pi^- + c.c.}
\newcommand{\gppkp}{\gamma \pi^+\pi^-K^+ \pi^- + c.c.}
\newcommand{\gksks}{\gamma K^0_s K^0_s}
\newcommand{\gphiphi}{\gamma \phi\phi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 6prongs
\newcommand{\tpp}{3(\pi^+\pi^-)}
\newcommand{\tppkk}{2(\pi^+\pi^-)(K^+K^-)}
\newcommand{\pptkk}{(\pi^+\pi^-)2(K^+K^-)}
\newcommand{\tkk}{3(K^+K^-)}
\newcommand{\gtpp}{\gamma 3(\pi^+\pi^-)}
\newcommand{\gtppkk}{\gamma 2(\pi^+\pi^-)(K^+K^-)}
\newcommand{\gpptkk}{\gamma (\pi^+\pi^-)2(K^+K^-)}
\newcommand{\gtkk}{\gamma 3(K^+K^-)}

%%************************************************************
%%  Variables and Formula
%%************************************************************
\newcommand{\psp}{\psi(3686)}
\newcommand{\jpsi}{J/\psi}
\newcommand{\ar}{\rightarrow}
\newcommand{\lra}{\longrightarrow}
\newcommand{\jpsito}{J/\psi \rightarrow }
\newcommand{\ptoppjp}{J/\psi \rightarrow\pi^+\pi^- J/\psi}
\newcommand{\pspto}{\psi^\prime \rightarrow }
\newcommand{\ptop}{\psi'\rightarrow\pi^0 J/\psi}
\newcommand{\ptoeta}{\psi'\rightarrow\eta J/\psi}
%\newcommand{\ptoeta}{\psi'\rightarrow
%\newcommand{\ptoeta}{\psi'\rightarrow
\newcommand{\ecto}{\eta_c \rightarrow }
\newcommand{\ecpto}{\eta_c^\prime \rightarrow }
\newcommand{\xto}{X(3594) \rightarrow }
\newcommand{\chicJto}{\chi_{cJ} \rightarrow }
\newcommand{\chiczto}{\chi_{c0} \rightarrow }
\newcommand{\chicoto}{\chi_{c1} \rightarrow }
\newcommand{\chictto}{\chi_{c2} \rightarrow }
\newcommand{\pspp}{\psi^{\prime\prime}}
\newcommand{\ptochic}{\psi(2S)\ar \gamma\chi_{c1,2}}
\newcommand{\ppjpsi}{\pi^0\pi^0 J/\psi}
\newcommand{\utoeta}{\Upsilon^{\prime}\ar\eta\Upsilon}
\newcommand{\ww}{\omega\omega}
\newcommand{\wf}{\omega\phi}
\newcommand{\ff}{\phi\phi}
\newcommand{\npsp}{N_{\psp}}
\newcommand{\llbpi}{\llb\pi^0}
\newcommand{\llbeta}{\llb\eta}
\newcommand{\ppi}{p\pi^-}
\newcommand{\pbpi}{\bar{p}\pi^+}
\newcommand{\lamb}{\bar{\Lambda}}
%%=================================================
%% abbreviated commands of LaTeX
%%=================================================
\def\ctup#1{$^{\cite{#1}}$}
\newcommand{\bfg}{\begin{figure}}
\newcommand{\efg}{\end{figure}}
\newcommand{\bitm}{\begin{itemize}}
\newcommand{\eitm}{\end{itemize}}
\newcommand{\bnum}{\begin{enumerate}}
\newcommand{\enum}{\end{enumerate}}
\newcommand{\btbl}{\begin{table}}
\newcommand{\etbl}{\end{table}}
\newcommand{\btbu}{\begin{tabular}}
\newcommand{\etbu}{\end{tabular}}
%\newcommand{\ol}{\overline}
\newcommand{\bcl}{\begin{center}}
\newcommand{\ecl}{\end{center}}
\newcommand{\bbt}{\bibitem}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqr}{\begin{eqnarray}}
\newcommand{\eeqr}{\end{eqnarray}}
%%===========================================
%%  color setting
%%===========================================
%\newcommand{\red}{\color{red}}
%\newcommand{\blue}{\color{blue}}
%\newcommand{\yellow}{\color{yellow}}
%\newcommand{\green}{\color{green}}
%\newcommand{\purple}{\color{purple}}
%\newcommand{\brown}{\color{brown}}
%\newcommand{\black}{\color{black}}
%%%============================================
%% mark
%%%============================================
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


